Assessing the Promise and Pitfalls of ChatGPT for Automated Code Generation

This paper presents a comprehensive evaluation of the code generation capabilities of ChatGPT, a prominent large language model, compared to human programmers. A novel dataset of 131 code-generation prompts across 5 categories was curated to enable robust analysis. Code solutions were generated by both ChatGPT and humans for all prompts, resulting in 262 code samples. A meticulous manual assessment methodology prioritized evaluating correctness, comprehensibility, and security using 14 established code quality metrics. The key findings reveal ChatGPT's strengths in crafting concise, efficient code with advanced constructs, showcasing strengths in data analysis tasks (93.1% accuracy) but limitations in visual-graphical challenges. Comparative analysis with human code highlights ChatGPT's inclination towards modular design and superior error handling. Additionally, machine learning models effectively distinguished ChatGPT from human code with up to 88% accuracy, suggesting detectable coding style disparities. By providing profound insights into ChatGPT's code generation capabilities and limitations through quantitative metrics and qualitative analysis, this study makes valuable contributions toward advancing AI-based programming assistants. The curated dataset and methodology offer a robust foundation for future research in this nascent domain. All data and codes are available on https://github.com/DSAatUSU/ChatGPT-promises-and-pitfalls.

==> tables/hyperparameters-table.tex <==
\begin{table}[htpb]\small
\label{tab:hyper}
\centering
\caption{Optimized hyperparameters after grid-search for the seven classification algorithm}
\label{table:hyperparameters-transposed}
\begin{tabularx}{\linewidth}{lX}
\toprule
\textbf{ML Algorithm} & \textbf{Hyperparameters} \\ \midrule

\multirow{2}{*}{Random Forest} & Criterion: Entropy, Max Depth: 50, Max Features: $\sqrt{}$, 
 Min Samples Leaf: 2, Min Samples Split: 2, N Estimators: 10, Random State: 803 \\ \hline
 
\multirow{2}{*}{Decision Tree} & Criterion: Entropy, Max Depth: 50, Max Features: $\sqrt{}$,  Min Samples Leaf: 2, Min Samples Split: 2, Splitter: Random, Random State: 8145 \\ \hline
 
\multirow{1}{*}{RUSBoost} & Algorithm: SAMME.R, Estimator: Logistic Regression, Learning Rate: 0.5, N Estimators: 50 \\ \hline
 
\multirow{1}{*}{Gaussian Naive Bayes} & Priors: None, Variance Smoothing: $1 \times 10^{-7}$ \\ \hline
 
\multirow{1}{*}{K-Nearest Neighbors} & Algorithm: Auto, Leaf Size: 10, Metric: Minkowski,  Num of Neighbors: 9, P: 4, Weights: Distance \\ \hline
 
\multirow{2}{*}{XGBoost} & Colsample Bytree: 0.8, Learning Rate: 0.01, Max Depth: 4, Min Child Weight: 4, Num of Estimators: 100, Subsample: 0.5 \\ \hline
 
\multirow{2}{*}{MLP} & Hidden Layer Sizes: (64, 32, 16), Max Iterations: 500, Alpha: 0.0001, Solver: Adam, Random State: 21, Tolerance: $1 \times 10^{-9}$ \\ \bottomrule
\end{tabularx}
\end{table}
